Stochastic Dissipativity for Systems with Probabilistic Input Delays

This work considers stochastic operators in general inner-product spaces, and in particular, systems with stochastically time-varying input delays of a known probability distribution. Stochastic dissipativity and stability are defined from an operator-theoretic perspective, and the well-known open-loop dissipativity conditions for closed-loop/network stability are extended to the stochastic case. Criteria are derived to identify dissipative nonlinear systems with stochastic input delays, and this result is used to find delay-distribution-dependent linear matrix inequality conditions for stochastic dissipativity of a linear system with input delays of a known probability distribution. A numerical experiment demonstrates the utility of the resulting criteria for robust plant analysis and controller design, highlighting significantly reduced conservatism compared to deterministic methods.

==> Backmatter.tex <==
\clearpage

\section*{Author Biography}

\begin{biography}{\includegraphics[width=66pt,height=86pt]{./Figures/EthanPicture.jpg}}{\textbf{Ethan J. LoCicero.} Ethan earned a B.S. in mechanical engineering from the University of Notre Dame, IN, USA in 2019. His undergraduate studies included research internships at Honeywell Aerospace Advanced Technology in South Bend, IN, and NASA Marshall Space Flight Center in Huntsville, AL. He is currently pursuing a Ph.D. in mechanical engineering at Duke University, Durham, NC. During his graduate studies, he interned at TerraPower in Bellevue, WA. Ethan also earned the 2019 Alfred P. Sloan Foundation Minority Ph.D. Scholarship, the 2021 NSF Graduate Research Fellowship, and the 2022 Burroughs Wellcome Fellowship. Ethan's dissertation research focuses on combining optimal control methods with nonlinear stability analysis to provide high performance and robust stability, especially for large-scale networks. Ethan's application interests include control of distributed energy resources, nuclear power generation, and autonomous vehicles.
}
\end{biography}

\begin{biography}{\includegraphics[width=66pt,height=86pt]{./Figures/Amy-Strong-Headshot-v2}}{\textbf{Amy K. Strong.} 
Amy Strong earned her B.M.E. and M.S. in Mechanical Engineering at Auburn University in 2018 and 2021 respectively. During her masters studies, she worked in the GPS and Vehicle Dynamics lab at Auburn University and interned at Sandia National Laboratories. She is currently pursuing her Ph.D. in Mechanical Engineering at Duke University in the Bridgeman Lab. While at Duke, Amy earned the Duke University Pratt-Gardner Graduate fellowship and the Burroughs Wellcome Fund fellowship. Additionally, she participated in the 2022-2023 NSF traineeship for the Advancement of Surgical Technologies. Her research interests include robust reinforcement learning, dissipativity, and medical robotics.}
%Amy K. Strong is a human doctoral student in the Department of Mechanical Engineering and Materials Science at Duke University, despite what her photo would have you believe. She is less furry in real life, and has a shorter tail. Amy earned B.Eng. and M.Eng. degrees (is that how Americans abbreviate them?) in Mechanical Engineering from Auburn University in the past. She also worked at a national lab. She is a great student, studying many topics that her supervisor knows about, but wants her to describe as she sees fit. It is taking an unexpected amount of effort to write text long enough to fill the space beside the photo. Be carfeful to crop your photo right. If your photo was originally 2400x3600, crop height to 3127.}
\end{biography}

\begin{biography}{\includegraphics[width=66pt,height=86pt]{./Figures/Leila_IJRNC.jpg}}{\textbf{Leila J. Bridgeman.} Leila Bridgeman earned B.Sc. and M.Sc. degrees in Applied Mathematics in 2008 and 2010 from McGill University, Montreal, QC, Canada, where she completed her Ph.D. in Mechanical Engineering, earning McGill’s 2016 D.W. Ambridge Prize for outstanding dissertation in the physical sciences and engineering. Her graduate studies involved research semesters at University of Michigan, University of Bern, and University of Victoria, along with an internship at Mitsubishi Electric Research Laboratories (MERL) in Boston, MA. She is now an assistant professor of Mechanical Engineering and Materials Science. Through her research, Leila explores how the tools of numerical analysis and input-output stability theory can be applied to the most challenging of controls problems, including the control of delayed, open-loop unstable, and nonminimum-phase systems.  Her focus has been on the development of readily applicable controller synthesis and stability analysis methods based on the evaluation of linear matrix inequalities (LMIs). Resulting publications have considered applications of this work to robotic, process control, and time-delay systems.
}
\end{biography}
